Online Time Series Anomaly Detection with State Space Gaussian Processes

We propose r-ssGPFA, an unsupervised online anomaly detection model for uni- and multivariate time series building on the efficient state space formulation of Gaussian processes. For high-dimensional time series, we propose an extension of Gaussian process factor analysis to identify the common latent processes of the time series, allowing us to detect anomalies efficiently in an interpretable manner. We gain explainability while speeding up computations by imposing an orthogonality constraint on the mapping from the latent to the observed. Our model's robustness is improved by using a simple heuristic to skip Kalman updates when encountering anomalous observations. We investigate the behaviour of our model on synthetic data and show on standard benchmark datasets that our method is competitive with state-of-the-art methods while being computationally cheaper.

==> sections/problem_statement.tex <==
%!TEX root = ../main.tex

\section{Problem Statement}
\label{sec:problem_statement}
Let $\vecVar{y}_{:, 1:T} = [\vecVar{y}_{:, 1}, \vecVar{y}_{:, 2}, \ldots, \vecVar{y}_{:, T}]$, denote a multivariate time series, where at each time point $t$%
\footnote{While our method is applicable to non-equally-spaced time series, we abuse notation and conflate time point and time index here to ease the exposition.}%
we have an observation vector $\vecVar{y}_{:, t} = [y_{1, t}, y_{2, t}, \ldots, y_{D, t}]^T \in \mathbb{R}^D$. Our goal is to decide for each $\vecVar{y}_{:, t}$ whether it is anomalous or not, determining the value of the binary \emph{anomaly indicator} variable $a_t \in \{0, 1\}$. In the online AD setting, observations arrive one at a time, and the anomaly decision for point $\vecVar{y}_{:, t}$ can be based only on observations up to and including that point. 

Following prior work \citep{ruff2020unifying}



Let us denote a $D$-dimensional time series $\B{t}$ of length $T$ as the sequence of pairs $\B{t}=(( \yvec_\timeVar, \avec_\timeVar))_{\timeVar=1}^{T}$.
%
%
Similarly, the \emph{measurement matrix} $\ymat \in \mathbb{R}^{D \times T}$ represents all measurements, possibly empty or imputed. We overload $t$ to be both the time point and the index of $ \yvec$ to simplify the notation.
%
Each observation is annotated by the  \emph{anomaly matrix} $\amat \in \{\varnothing,0,1\}^{d \times n}$, where $1$ annotates anomalies,  $0$  non-anomalies, and $\varnothing$ unlabelled observations.
%
Due to the unlikely nature of anomalies and the high costs of receiving ground truth labels, data sets are commonly dominated by unlabelled observations requiring unsupervised learning approaches.

x the unknown \emph{ground truth law of normal behaviour}. The data is corrupted by anomalies drawn from $\mathbb{P}^-$. We aim at detecting these corrupted points by learning the temporal behaviour of $ \mathbb{P}^+$ and detect unlikely points under this distribution.




\iffalse
In the streaming setting, we are interested in obtaining anomaly scores for a potentially infinitely long stream of data in real-time. The following aspects make this setup particularly challenging:
\begin{enumerate*}
	\item Inference time: Anomaly scores should be efficiently computable,
	\item space complexity: The model's memory requirements should not scale with the length of the~(potentially infinite) data stream, 
	\item the aforementioned distribution shift~(e.g.\ through a change in units of a measurement) should be accounted for, and
	\item cold-start scenario: $n_\text{train}$ can be very small or even zero.
\end{enumerate*}


\paragraph{What are Time Series Anomalies?}
% The definition of what constitutes an anomaly is non-trivial. An ontology which differentiates between \emph{point}, \emph{contextual}, and \emph{collective} anomalies has emerged~\citep{chandola2009anomaly}. 
%
In this work, we define time series anomalies as \emph{low probability} observations or sequences of observations as measured against a predictive distribution. 
%
The \emph{exptected} behaviour is governed by an unknown dynamical process whose external interruption is manifested in anomalies.
%
We assume that the underlying process is of stochastic nature and model it as a Gaussian Process~\citep{gp_for_ml}.

\fi



\iffalse
\paragraph{Offline Anomaly Detection~(O-AD)}
\todo[inline]{M: Offline AD model keeps unchanged, but isn't inference still based on new data? We need more work on it}
Given  a set of $n_{\text{train}}$ training observations $T_{\text{train}} = ((\tvec_\timeVar, \yvec_\timeVar))_{\timeVar=1}^{n_{\text{train}}}$, the objective in offline anomaly detection is to predict the correct  \emph{anomaly matrix} $\matVar{A}_\text{test} \in \{0,1\}^{d \times n_\text{test}}$, where $n_\text{test}$ is the length of the test sequence.
\todo[inline]{M: We need to describe learnable model and predict $\matVar{A}_\text{test} | (\tvec_\text{test}, \yvec_\text{test})$. L: we state in the intro that we focused on unsupervised models so maybe just skip that.}
%
Although the correct~(binary) prediction of $\matVar{A}$ can be the desired solution, in practice, it is scored by  \emph{anomaly scores}, which describe the degree of anomality of a given observation. If we denote anomaly scoring function $l$, thus, 
\begin{equation}
	\label{eq:anomaly score}
	P(l(\tvec_\text{test}, \yvec_\text{test}) > \alpha) < \beta
\end{equation}

where $\beta$ is arbitrary small number, and $\alpha$ is specific threshold to determine whether it is anomaly score or not. 
% 
When this is the case, and for the remainder of this paper, $\matVar{A}_\text{test} \in \mathbb{R}^{d \times n_\text{test}}$.
%
While O-AD methods enjoy the property of ``train once, use repeatedly'', a drawback of these approaches is their inability to adapt to changing data distributions~(e.g.\ change-points). \todo[inline]{M: this may not be true if we detect anomalies in batches, these batches could be treated partial of training dataset. (There are mulitple offline change-point algorithms, https://arxiv.org/pdf/1801.00718.pdf)}
%
\todo[inline]{M: One of benefit of offline method, you can leverage information based on history and future, it has better results but \emph{costly} in nature}
While frequent retraining could be a remedy for this problem, it is a costly procedure and requires building a decision procedure to trigger the retraining and decide on the amount of data to consider in the retraining.
%
Furthermore, the computational cost of model retraining~(especially when using large neural networks) can be prohibitive, emphasizing the practical utility of O-AD methods under distribution shifts. 
\fi




